Space4HGNN: A Novel, Modularized and Reproducible Platform to Evaluate Heterogeneous Graph Neural Network

Heterogeneous Graph Neural Network (HGNN) has been successfully employed in various tasks, but we cannot accurately know the importance of different design dimensions of HGNNs due to diverse architectures and applied scenarios. Besides, in the research community of HGNNs, implementing and evaluating various tasks still need much human effort. To mitigate these issues, we first propose a unified framework covering most HGNNs, consisting of three components: heterogeneous linear transformation, heterogeneous graph transformation, and heterogeneous message passing layer. Then we build a platform Space4HGNN by defining a design space for HGNNs based on the unified framework, which offers modularized components, reproducible implementations, and standardized evaluation for HGNNs. Finally, we conduct experiments to analyze the effect of different designs. With the insights found, we distill a condensed design space and verify its effectiveness.

==> Input/Condensed.tex <==

\section{Evaluation of Condensed Design Space}

Section~\ref{experiments} reveals that it is hard to design a single HGNN model that can guarantee outstanding performance across diverse scenarios in the real world. Motivated by \cite{radosavovic2019network, radosavovic2020designing}, focusing on design space that consists of a collection of models instead of individual architecture brings more generalization and robustness. According to the findings in Section\ref{exp:common_design}, we condensed the design space to facilitate model searching. Specifically, we remove some bad choices in design dimensions and retain some essential design dimensions (e.g., high-level architectural structures and helpful design principles).
\subsection{The Condensed Design Space}
For common design dimensions with GraphGym, Table~\ref{tab:condensed} compares the condensed design spaces we and GraphGym proposed. We retain some of the design dimensions same as GraphGym if the findings in Section~\ref{exp:common_design} are aligned (i.e., layer connectivity, optimizer, and training epochs).  We propose our own choices for the different dimensions in conclusion (e.g., Dropout, activation, BN, L2-Norm, etc.).
%Following some findings specific to HGNN, we have a minor modification to some design dimensions (e.g., dropout, activation, and pre-process layers). Besides, there are some non-negligible results in task-wise evaluation, and we retained all choices for BN and L2-Norm.
For unique design dimensions in HGNN, we conclude that the micro-aggregation and model family design dimensions vary greatly across datasets or tasks. So we retain all choices in unique design dimensions and aim to find out whether the variants of existing HGNNs could gain improvements in HGB.

The original design space contains over 40M combinations, and the condensed design space contains 70K combinations. So the possible combination of the design dimensions in condensed design space is reduced by nearly 500 times.


\subsection{Evaluation of Different Design Spaces}
Plotting ranking with controlled random search can only work in the same design space, and is not suitable for evaluation across different design spaces.  Therefore, we plot for each design space the empirical distribution function (EDF) \cite{radosavovic2019network}: given $n$ configurations and their respective scores $s_i$, EDF is defined as
\begin{equation}
F(s)=\frac{1}{n} \sum_{i=1}^{n} \mathbf{1}\left[s_{i}<s\right].
\end{equation}
EDF essentially tells the probability of a random hyperparameter configuration that \emph{cannot} achieve a given performance metric.  Therefore, with $x$-axis being the performance metric and $y$-axis being the probability, an EDF curve closer to the lower-right corner indicates that a random configuration is more likely to get a better result.

\begin{table}[htpb]
    \centering
    \caption{Condensed common design dimensions with GraphGym.  Unique dimensions in HGNNs are not condensed.}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c|c}
    \toprule
       \textbf{Design Dimension} & \textbf{\makecell[c]{Our Condensed \\Design Space}} & \textbf{\makecell[c]{Condensed Design Space\\ in GraphGym}} \\
    \midrule
        Batch Normalization & True, False & True\\
        Dropout & 0, 0.3 & 0 \\
        Activation & ELU LeakyReLU Tanh & PReLU \\
        L2 Normalization & True, False &  - \\
    \midrule
        Layer Connectivity & SKIP-SUM, SKIP-CAT & SKIP-SUM, SKIP-CAT \\
        Pre-process Layers & 1 & 1, 2\\
        Message Passing Layers & 1, 2, 3, 4, 5, 6 & 2, 4, 6, 8\\
        Post-process Layers & 1, 2 & 2, 3\\
    \midrule
        Optimizer & Adam & Adam\\
        Learning Rate & 0.1, 0.01 & 0.01\\
        Training Epochs & 400 & 400\\
        Hidden dimension & 64, 128 & -\\
    \bottomrule
    \end{tabular}}
    \label{tab:condensed}
\end{table}
% Another comparison paradigm is distribution estimates \cite{radosavovic2019network}. And different design spaces can be compared with a distribution curve as shown in Fig~\ref{fig:dis_dataset}. To compare distributions, we use empirical distribution functions (EDFs). Let $\mathbf{1}$ be the indicator function. Given a set of $n$ models with scores {$s_{i}$}, the score EDF is given by:

% \begin{equation}
% F(e)=\frac{1}{n} \sum_{i=1}^{n} \mathbf{1}\left[s_{i}<s\right].
% \end{equation}

% $F(e)$ gives the fraction of models with score less than $s$. In our design space, each model family corresponds to a subspace and can be compared by distribution estimate.

% In addition to plotting the average ranking and the distribution of rankings like \cite{you2020design} for individual design space dimensions, we also consider comparing the models with distribution estimates \cite{radosavovic2019network} 
Though the condensed design space in GraphGym is small enough to perform a full grid search for GNNs, it is not so much suitable for HGNNs due to more complicated HGNN models. To verify the effectiveness of our condensed design space, we compare it with the original design space and the condensed design from GraphGym \cite{you2020design}. We randomly search 100 designs in three spaces, respectively.

As shown in Figure~\ref{fig:condensed_dis}, our condensed design space outperforms the others. Specifically, the original design space has many bad choices (i.e., optimizer with SGD) and performs worst in the distribution estimates. On the other hand, the best design in the original design space is competitive, but at a much higher search cost.  %not so bad, which means random search in the original design space could get a not so bad result but cost too much.
Besides, the better performance in our condensed design space compared with GraphGym shows that we cannot simply transfer the design space condensed from homogeneous graphs to HGNNs, and specific condensation is required.%it is imperative to define design space for HGNN and distill specific findings in HGNNs. 
\begin{table*}[htpb]
    \caption{Comparison with the standard HGNNs in HGB. The prefix HGBn means dataset of node classification and the prefix HGBl means dataset of link prediction. Vacant positions (-) are due to lack of baselines in HGB. The lower average rank is better.}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|cc|cc|cc|cc|cc|c}
    \toprule
         & \multicolumn{2}{c|}{HGBn-DBLP} & \multicolumn{2}{c|}{HGBn-ACM} &\multicolumn{2}{c|}{HGBl-amazon} &\multicolumn{2}{c|}{HGBl-LastFM}  \\
    \midrule
         & Macro-F1 & Micro-F1 & Macro-F1 & Micro-F1 & ROC-AUC & MRR & ROC-AUC & MRR  & Average Rank\\
    \midrule
        GCN & 90.84$\pm0.32$ & 91.47$\pm0.34$ & 92.17$\pm0.24$ & 92.12$\pm0.23$ & 92.84$\pm0.34$ & \textbf{97.05$\pm0.12$} & 59.17$\pm0.31$ & 79.38$\pm0.65$ & 3.75\\
    \midrule
        GAT & 93.83$\pm0.27$ & 93.39$\pm0.30$& 92.26$\pm0.94$ & 92.19$\pm0.93$ & 91.65$\pm0.80$ & 96.58$\pm0.26$ & 58.56$\pm0.66$ & 77.04$\pm2.11$ & 3.63\\
    \midrule
        RGCN & 91.52$\pm0.50$ & 92.07$\pm 0.50$ & 91.55$\pm 0.74$ & 91.41$\pm 0.75$ & 86.34$\pm0.28$& 93.92$\pm0.16$ & 57.21$\pm0.09$ & 77.68$\pm0.17$ & 5.13\\
    \midrule
        HAN & 91.67$\pm0.49$ & 92.05$\pm0.62$&  90.89$\pm 0.43$ & 90.79$\pm0.43$ & - & - & - & - & 6.63\\
    \midrule
        HGT & 93.01$\pm0.23$ &93.49$\pm0.25$ &91.12$\pm0.76$ &91.00$\pm0.76$& 88.26 $\pm2.06$ & 93.87 $\pm0.65$ & 54.99$\pm0.28$ & 74.96 $\pm1.46$ & 5.25\\
    \midrule
        Simple-HGN & 94.01$\pm0.24$ & 94.46$\pm 0.22$ & \textbf{93.42$\pm$0.44} & \textbf{ 93.35$\pm$0.45} & 93.49 $\pm0.62$ & 96.94$\pm0.29$ & 67.59$\pm0.23$ & 90.81$\pm0.32$ & 1.75\\
    \midrule
        Ours & \textbf{94.24$\pm$0.42} & \textbf{94.63$\pm$0.40}& 92.50 $\pm$0.14& 92.38$\pm$0.10& \textbf{95.15$\pm$0.43} & 96.56$\pm0.29$ & \textbf{70.15$\pm$0.77} & \textbf{91.12$\pm$0.38} & \textbf{1.63} \\
    \bottomrule
    \end{tabular}}
    \label{tab:NC_performance}
\end{table*}

\begin{table*}[]
    \centering
    \caption{Best designs in HGB, found by a simple random search in our condensed design space. }
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \toprule
        Dataset & Model Family & \makecell[c]{Micro-\\aggregation} & \makecell[c]{Macro-\\aggregation} & BN & L2-Norm & Dropout & Activation& \makecell[c]{Layer\\Connectivity} & \makecell[c]{Message\\Passing\\Layers} & \makecell[c]{Post-\\process \\Layers} \\
    \midrule
        HGBn-ACM & Relation & GCNConv & Sum & False & True & 0.0 & Tanh & SKIP-SUM & 2 & 2 \\
        HGBn-DBLP & Homogenization & GATConv & - & True & True & 0.0 & LeakyRelu & SKIP-SUM & 3 & 2\\
        HGBl-amazon & Meta-path & GATConv & Attention & True & False & 0.0 & LeakyRelu & SKIP-SUM & 5 & 1 \\
        HGBl-LastFM & Homogenization & SageConv & - & True & False & 0.3 & Elu & SKIP-CAT & 5 & 2 \\
    \bottomrule
    \end{tabular}}
    \label{tab:best_design}
\end{table*}
\subsection{Comparison with GraphNAS}
We also apply a GNN neural architecture search method GraphNAS \cite{graphnas} in the original design space as a comparison. The NAS is to find the best architecture, so we only report the best performance of GraphNAS in Figure~\ref{fig:condensed_dis}. Though GraphNAS outperforms in HGBn-DBLP and gains excellent performance in HGBl-ACM and HGBl-IMDB, it performs worst in other datasets. So compared with GraphNAS, our design space has more significant  advantages in robustness and stability. We think that we need a more advanced NAS method (i.e., DiffMG \cite{diffmg}) for our design space in future work.
%and the sub-optimal region can be removed
% It enables us to conduct a full grid search for further evaluation. Specifically, the condensed HGNN design space is shown in Table~\ref{tab:condensed}. And based on the condensed design space, we evaluate the three model families in Table~\ref{tab:dimension} in depth. Specifically, we use score EDF, which is introduced in Section~\ref{eva:comp}, to evaluate the performance distribution of the three paradigms on seven HGB datasets. The distribution estimate results are shown in Fig.~\ref{fig:node_dis}, where the top is the result of the original design space and the bottom is that of the condensed one.

% \subsubsection{Efficacy of the Condensed HGNN Design Space}
% We first compare the distribution estimates of the HGNN design space before and after being condensed on the same dataset. It can be observed on almost all datasets that the plots at the bottom are more sharp and their maximum values on the X-axis are smaller than that at the top. It reveals that although the highest score drops, the performance of the models in the condensed space still distributes in a high-scored area closely. Therefore, it is more efficient to find a model with relatively good performance, which facilitates our further evaluation and other model design. 

% \subsubsection{Distribution Estimate of Aggregation Paradigm Design}
% \label{AggPa}
% As the most important dimension of our HGNN design space, the influences of different aggregation paradigms should be analyzed in detail. 
% Then, with the condensed design space, we can perform a full grid search for three paradigms and evaluate their performance. By analyzing the results shown in Figure~\ref{fig:node_dis}, we hope to answer the following two questions:
% \begin{itemize}
%     \item \textbf{Q1: Is meta-path always favorable?} The answer is it depends. We can observe from Figure ~\ref{fig:node_dis} that none of the three paradigms consistently outperforms. When it comes to meta-path, in datasets such as HGBn-ACM and HGNn-DBLP where some informative and effective meta-paths have been empirically discovered, the meta-path paradigm outperforms the other two alternatives. However, in other datasets, its effectiveness is limited. It reminds us that meta-path should be delicately designed and exploited.
%     \item \textbf{Q2: Are we really making much progress in HGNN?}  \quan{Incomplete.}
% \end{itemize}
% \textbf{We hope to answer the question: are we really making much progress in HGNN?}

% According to Section ~\ref{common_design}, we prunes the original dimensions and fix several dimensions. With a condensed design space, we can perform a full grid search for three paradigms and analyze the performs of different paradigm. As shown in Figure ~\ref{fig:node_dis}, the top is the distribution estimate of the proposed design space and the bottom is the distribution of condensed sapce.
% Overall, the figure below has a steeper curve than the one above which means a condensed space bring an more efficient way to find not bad performance.

% \textbf{Does meta-path paradigm outperform?} In dataset HGBn-ACM and HGBn-DBLP, the meta-paths is significantly better. In the sampled models distribution estimate, the meta-path paradigm curve is 
% below the other two, which means you can find a high performance better. The bottom of ~\ref{fig:node_dis} shows a steeper slope than the top

% we implement several popular HGNNs using the Space4HGNN platform while controlling all the other dimensions the same as those in the condensed design space, and compare their performance with their counterparts reported by HGB on node classification and link prediction tasks. 
% \begin{table*}[htpb]
%     \caption{Caption}
%     \centering
%     \begin{tabular}{c|c|c|c|c}
%     \toprule
%         Model Family & \multicolumn{4}{c|}{amazon} \\
%     \midrule
%         & all-max & all-mean & \makecell[c]{condensed \\max} & \makecell[c]{condensed \\mean} \\
%     \midrule
%         Homogenization & \\
%         Relation & \\
%         Meta-path & \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:my_label}
% \end{table*}

% \begin{table*}[htpb]
%     \caption{Comparing with baselines in HGB. The prefix HGBn means dataset of node classification and the prefix HGBl means dataset of link prediction. Vacant positions (-) are due to lack of baselines in HGB.}
%     \centering
%     \resizebox{2\columnwidth}{!}{
%     \begin{tabular}{c|cc|cc|cc|cc|cc|c}
%     \toprule
%          & \multicolumn{2}{c|}{HGBn-DBLP} & \multicolumn{2}{c|}{HGBn-IMDB} & \multicolumn{2}{c|}{HGBn-ACM} &\multicolumn{2}{c|}{HGBl-amazon} &\multicolumn{2}{c|}{HGBl-LastFM}  \\
%     \midrule
%          & Macro-F1 & Micro-F1 & Macro-F1 & Micro-F1 & Macro-F1 & Micro-F1 & ROC-AUC & MRR & ROC-AUC & MRR  & Average Rank\\
%     \midrule
%         GCN & 90.84$\pm0.32$ & 91.47$\pm0.34$ & 57.88$\pm1.18$ & 64.82$\pm0.64$ & 92.17$\pm0.24$ & 92.12$\pm0.23$ & 92.84$\pm0.34$ & \textbf{97.05$\pm0.12$} & 59.17$\pm0.31$ & 79.38$\pm0.65$\\
%         % GCN(ours) & 90.93$\pm1.23$ & 91.78$\pm1.03$& 61.85$\pm0.25$ & 65.18$\pm0.37$& 91.30$\pm0.25$& 91.27$\pm0.24$ & 93.30$\pm1.35$&96.06$\pm0.24$ & 67.58$\pm1.30$ & 90.31$\pm0.53$ \\
%     \midrule
%         GAT & 93.83$\pm0.27$ & 93.39$\pm0.30$ & 58.94$\pm1.35$ & 64.86$\pm0.43$ & 92.26$\pm0.94$ & 92.19$\pm0.93$ & 91.65$\pm0.80$ & 96.58$\pm0.26$ & 58.56$\pm0.66$ & 77.04$\pm2.11$ \\
%         % GAT(ours) & 93.63$\pm0.42$ & 94.09 $\pm0.41$ & 62.06$\pm0.62$ & 65.26 $\pm0.84$ & 89.70 $\pm0.70$ &89.68$\pm0.69$ & 92.81$\pm1.12$ & 94.88 $\pm0.66$& 65.62$\pm0.80$ & 87.01$\pm1.01$\\
%     \midrule
%         RGCN & 91.52$\pm0.50$ & 92.07$\pm 0.50$ & 58.85$\pm 0.26$ & 62.05$\pm 0.15$ & 91.55$\pm 0.74$ & 91.41$\pm 0.75$ & 86.34$\pm0.28$& 93.92$\pm0.16$ & 57.21$\pm0.09$ & 77.68$\pm0.17$ \\
%         % RGCN(ours) & 93.20$\pm1.83$ & 93.64$\pm1.84$ & 60.07 $\pm2.23$ & 64.28 $\pm2.04$ & 89.79$\pm1.21$& 89.70$\pm1.23$ & 89.25$\pm0.54$& 94.42$\pm0.51$ & 61.96$\pm0.91$ & 87.02$\pm1.24$ \\
%     \midrule
%         HAN & 91.67$\pm0.49$ & 92.05$\pm0.62$ & 57.74$\pm0.96$ & 64.63$\pm0.58$ &  90.89$\pm 0.43$ & 90.79$\pm0.43$ & - & - & - & -\\
%         % HAN(ours) & 92.50 $\pm0.13$ & 92.99 $\pm0.11$ & 59.67 $\pm1.54$ & 62.16 $\pm1.30$ & 90.80 $\pm0.36$ & 90.70 $\pm0.35$& 93.93$\pm0.37$ & 96.28$\pm0.31$ & 62.88$\pm1.39$ & 88.22 $\pm0.58$\\
%     \midrule
%         HGT & 93.01$\pm0.23$ &93.49$\pm0.25$ & 63.00$\pm1.19$&67.20$\pm0.57$&91.12$\pm0.76$ &91.00$\pm0.76$& 88.26 $\pm2.06$ & 93.87 $\pm0.65$ & 54.99$\pm0.28$ & 74.96 $\pm1.46$ \\
%         % HGT(ours) & 91.10 $\pm1.86$& 91.97 $\pm1.41$ & 63.34$\pm0.46$ & 65.10$\pm0.54$ & & & & & 54.72$\pm1.47$ & 82.73 $\pm0.27$ \\
%     \midrule
%         Simple-HGN & 94.01$\pm0.24$ & 94.46$\pm 0.22$ & 63.53$\pm1.36$ & 67.36$\pm0.57$ & 93.42$\pm0.44$ & 93.35$\pm0.45$ & 93.49 $\pm0.62$ & 96.94$\pm0.29$ & 67.59$\pm0.23$ & 90.81$\pm0.32$\\
%         % Simple-HGN(ours) &94.23 $\pm0.17$ & 94.65$\pm0.15$ &62.89$\pm0.30$ & 65.71$\pm0.34$ & & &92.07 $\pm1.09$ & 93.26$\pm0.44$ & 64.48$\pm1.26$ &88.74$\pm0.51$ \\
%     % \midrule
%     %     homo &94.24$\pm0.42$ &94.63$\pm0.40$ & 60.97$\pm3.13$ &65.58$\pm0.93$ & 88.02$\pm0.59$ & 87.92$\pm0.62$ & 94.11$\pm0.64$ & 95.96 $\pm0.15$ & 67.53 $\pm2.09$ & 90.00 $\pm0.15$ \\
%     %     meta-path &93.12$\pm0.30$ &93.63$\pm0.28$ & 61.39$\pm0.26$ & 64.90$\pm0.28$ &89.62$\pm0.21$ &89.46$\pm0.22$ & 95.15$\pm0.43$ & 96.56$\pm0.29$ & 68.68$\pm0.43$ & 90.77$\pm0.22$ \\
%     %     relation &93.32$\pm0.22$ & 93.80$\pm0.24$ & 61.47$\pm0.26$ & 65.13$\pm0.04$ &91.78$\pm0.30$ &91.68$\pm0.30$ & 93.53$\pm1.07$ & 96.46 $\pm0.29$ & 66.36$\pm1.43$ & 87.01$\pm0.56$ \\
%     \midrule
%         ours & \textbf{94.24$\pm$0.42} & \textbf{94.63$\pm$0.40} & 61.85$\pm0.25$ & 65.18$\pm0.37$& 92.50 $\pm$0.14& 92.38$\pm$0.10& \textbf{95.15$\pm$0.43} & 96.56$\pm0.29$ & \textbf{70.15$\pm$0.77} & \textbf{91.12$\pm$0.38} \\
%     \bottomrule
%     \end{tabular}}
%     \label{tab:NC_performance}
% \end{table*}

\subsection{Evaluation in Heterogeneous Graph Benchmark (HGB)}
To compare with the performance of the standard HGNNs, we evaluate our condensed design space in a new benchmark HGB. We randomly searched 100 designs from condensed design space and evaluated the best design of validation set in HGB. As shown in Table~\ref{tab:NC_performance}, our designs with condensed design space can achieve comparable performance. So we can easily achieve SOTA performance with a simple random search in the condensed design space. Table~\ref{tab:best_design} shows the best designs we found in our condensed design space, which cover the variants of RGCN and HAN. It also confirms that the meta-path model family and the relation model family have great performance in HGB and further answers the question \emph{``are meta-path or variants still useful in GNNs?"} from \cite{Simple-HGN}.
Note that this result does not contradict the conclusion from \cite{Simple-HGN}, as our design space includes much more components than the vanilla RGCN or HAN model, and proper components can make up shortcomings of an existing model.
%Our work does not conflict with the work \cite{Simple-HGN} that has a worrying doubt on progress of HGNN, and we aim to advance the developments of HGNN with design space. Our design space for HGNN makes up for the shortcomings of a single model, and verifies the effect of design architecture of existing HGNN models.
% \subsection{Case Study: Scoring Function as a New Design Dimension} \label{case_study}
% As mentioned in Section \ref{space4hgnn}, we offer a platform to encourage the researchers to flexibly adjust the design space by adding new design dimensions and removing unneeded ones.

% Here, we provide a case study, where we investigate the \textit{Scoring Function} as a new design dimension for the link prediction task. Compared to the commonly used dot product, HGB prefers DistMult ~\cite{yang2014embedding} as the scoring function to predict the probability of the existence of an edge for a given node pair even when there is only single type of edge to predict. Based on our design space, we compare the HGNN performance with dot product or DistMult as the scoring function for the link prediction task. As shown in Fig.~\ref{fig:score_fn}, we can observe that dot product
% dot product can achieve better performance more stably than DistMult from the right rank analysis. From the right distribute estimate, DistMult is better in high performance part which is consistent with the claim in ~\cite{Simple-HGN}.

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{images/score_fn.png}
%     \caption{Rank and distribute estimate for score function in link prediction. The left is rank analysis. The right is distribute estimate and the bottom is the an enlarged version of the higher performance part of the top.}
%     \label{fig:score_fn}
% \end{figure}

% Although we define an effective HGNN design space which can cover a variety of HGNN architectures, it should be emphasized that our aim is not to pursue the most complex combinations of as many design dimensions as possible. New scenarios are appearing and we wonder whether new techniques work in new scenarios. Subsequently, we offer a platform to encourage the researchers to flexibly adjust the design space by adding new design dimensions and removing unneeded ones.

% \begin{table*}[htpb]
%     \centering
%     \begin{tabular}{c|cc|cc|cc}
%     \toprule
%          & \multicolumn{2}{c}{HGBl-amazon} & \multicolumn{2}{c}{HGBn-LastFM} & \multicolumn{2}{c}{HGBn-PubMed} \\
%     \midrule
%          & ROC-AUC & MRR & ROC-AUC & MRR & ROC-AUC & MRR \\
%     \midrule
%         GCN & 92.84$\pm0.34$ & 97.05$\pm0.12$ & 59.17$\pm0.31$ & 79.38$\pm0.65$ & 80.48$\pm0.81$ & 90.99$\pm0.56$ \\
%         GCN(ours) & 90.25$\pm0.78$&93.35$\pm0.08$ & 63.97$\pm1.68$ & 87.88$\pm0.77$ & 86.80$\pm0.06$ & 90.05$\pm0.03$ \\
%     \midrule
%         GAT & 91.65$\pm0.80$ & 96.58$\pm0.26$ & 58.56$\pm0.66$ & 77.04$\pm2.11$ & 78.05$\pm1.77$ & 90.02$\pm0.26$ \\
%         GAT(ours) & 91.50$\pm$0.57 & 93.45 $\pm0.30$& 60.89$\pm2.90$ & 86.58$\pm0.86$\\
%     \midrule
%         RGCN & 86.34$\pm0.28$& 93.92$\pm0.16$ & 57.21$\pm0.09$ & 77.68$\pm0.17$ & 78.29$\pm0.18$ & 90.26 $\pm0.24$ \\
%         RGCN(ours) & 84.53$\pm1.17$& 91.36$\pm0.19$ & 79.67$\pm1.23$ & 81.61$\pm1.07$ & & \\
%     \midrule
%         HAN(ours) & & & 54.72$\pm1.47$ & 82.73 $\pm0.27$\\
%     \midrule
%         Simple-HGN & 93.49 $\pm0.62$ & 96.94$\pm0.29$ & 67.59$\pm0.23$ & 90.81$\pm0.32$ &83.39 $\pm0.39$ & 92.07$\pm0.26$\\
%         Simple-HGN(ours) & 92.07 $\pm1.09$ & 93.26$\pm0.44$ & 64.48$\pm1.26$ &88.74$\pm0.51$ \\
%     \bottomrule
%     \end{tabular}
%     \caption{Link Prediction}
%     \label{tab:LP_performance}
% \end{table*}


==> Input/Design_Space.tex <==


\section{Design Space}
As illustrated in Figure~\ref{fig:design}, we define a design space for HGNNs and describe it from two aspects: common designs with GraphGym and unique designs distilled from HGNNs. Though GraphGym \cite{you2020design} distills guidelines for designing well-performing GNNs, we still design the related dimensions to figure out whether they are still effective in HGNNs. However, the dimensions used in GNNs are not enough to design space for HGNN, and there are some unique dimensions in HGNNs. According to the unified framework proposed above, we propose three HGNN model families, which can reproduce most original HGNN models and extend new variants by applying different choices in unique dimensions. To highlight their roles in HGNNs, we design three corresponding sub-spaces for the three model families, which are homogenization model family, relation model family and meta-path model family. Besides, our design space is built as a platform offering modularized HGNN implementation for researchers introduced at last.   
% \quan{So our design space will indeed not cover HGT and Simple-HGN?  That's OK.  However, "well-designed" sounds positive, thus will make people wonder why you don't cover it.  I guess "unique" or "uniquely handcrafted" because you want to emphasize all those attentions are different?}.
% \quan{Consider move the last sentence up before "Our space will not contain ..." as the omission is not what we define for design space.}

\begin{figure*}[htpb]
    \centering
    \includegraphics[width=\textwidth]{images/spacev5.png}
    \caption{Design space: (1) The red and yellow font represents the design dimension and the blue font means choice of model families. (2) The red dotted frame includes the dimensions of the unique design in HGNNs. And blue dotted frame indicates some common dimensions with GraphGym.}
    \label{fig:design}
\end{figure*}

\begin{table}[h]
    \caption{Common design dimensions with GraphGym.}
    \begin{center}
    % \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c}
    \toprule
       \textbf{Design Dimension} & \textbf{Choices} \\
    % \midrule
    %     Paradigm & Homogenization, Relation, Meta-path \\
    %     \makecell[c]{Convolution \\ Micro-level Aggregation} & GCNConv, GATConv, SageConv, GINConv\\
    %     Macro-level Aggregation & Mean, Max, Sum, Attention \\
    \midrule
        Batch Normalization & True, False \\
        Dropout & 0, 0.3, 0.6 \\
        Activation & Relu, LeakyRelu, Elu, Tanh, PRelu \\
        L2 Normalization & True, False \\
    \midrule
        Layer Connectivity & STACK, SKIP-SUM, SKIP-CAT \\
        Pre-process Layers & 1, 2, 3 \\
        Message Passing Layers & 1, 2, 3, 4, 5, 6\\
        Post-process Layers & 1, 2, 3 \\
    \midrule
        Optimizer & Adam, SGD \\
        Learning Rate & 0.1, 0.01, 0.001, 0.0001 \\
        Training Epochs & 100, 200, 400 \\
        Hidden dimension & 8, 16, 32, 64, 128 \\
    \bottomrule
    \end{tabular}
    \label{tab:dimension}
    \end{center}
\end{table}
\subsection{Common Designs with GraphGym}
The common designs with GraphGym involves 12 design dimensions, categorized three aspects, intra-layer, inter-layer and training settings. The dimensions with corresponding choices are shown in Table~\ref{tab:dimension}.

\subsubsection{Intra-layer}
Same with GNNs, an HGNN contains several Heterogeneous GNN layers, where each layer could have diverse design dimensions. As illustrated in Figure~\ref{fig:design}, the adopted Heterogeneous GNN layer has an aggregation layer which involves unique design dimensions discussed later, followed by a sequence of modules: 
(1) batch normalization BN($\cdot$) \cite{BN}; 
(2) dropout DROP($\cdot$) \cite{dropout}; 
(3) nonlinear activation function ACT($\cdot$); 
(4) L2 Normalization L2-Norm($\cdot$). 
Formally, the L-th heterogeneous GNN layer can be defined as:
% \begin{equation}
% \begin{aligned}
% \mathbf{h}_{v}^{(L+1)}=\operatorname{Inter-layer}( \operatorname{AGG}\left\{\mathbf{h}_{u}^{(L)}, u \in \mathcal{N}_{v})\right\}),
% \end{aligned}
% \end{equation}

% \begin{equation}
%     \operatorname{Inter-layer(\cdot)} = \operatorname{L2-Norm}\left(\operatorname{ACT}\left(\operatorname{DROP}\left(\operatorname{BN}\left( \cdot \right)\right)\right)\right).
% \end{equation}
\begin{small}
\begin{equation}
\begin{aligned}
\mathbf{h}_{v}^{(L+1)}=\operatorname{L2-Norm}\left(\operatorname{ACT}\left(\operatorname{DROP}\left(\operatorname{BN}\left(
\operatorname{AGG}\left\{\mathbf{h}_{u}^{(L)}, u \in \mathcal{N}_{v})\right\}
\right)\right)\right)\right).
\end{aligned}
\end{equation}
\end{small}

\subsubsection{Inter-layer}
The layers of message passing, pre-processor and post-processor are supposed to be considered, which are essential design dimensions according to empirical evidence from neural networks. The HGNN layers iteratively transform features, resulting in the problems of vanishing gradient, over-fitting and over-smoothing, and the last problem is seen as the obstacles to stack deeper GNN layers. Inspired by ResNet \cite{resnet} to alleviate the problems, skip connection \cite{deepgcns, xu2018representation} has been proven to significant effect. Following \cite{you2020design}, we investigate two choices of skip connections: SKIP-SUM \cite{resnet} and SKIP-CAT \cite{huang2017densely} with STACK as a basic comparison.
    
\subsubsection{Training Settings}
As a part of deep learning, we also want to analyze design dimensions on training settings, like optimizer, learning rate and training epochs. Besides, the hidden dimension is also included here involving the trainable parameters.

\subsection{Unique Design in HGNNs} \label{aggregation paradigm}
With the unified framework, we try to transform the modular components into unique design dimensions in HGNNs. According to \cite{radosavovic2019network}, a collection of related neural network architectures, typically sharing some high-level architectural structures or design principles (e.g., residual connections), could be abstracted into a model family. With that, we distill three model families in HGNNs. As shown in Table~\ref{tab:model families}, three model families involve three design dimensions with candidate choices.

% \begin{table}[h]
%     \caption{Three model families with corresponding sub-space}
%     \begin{center}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{c|c|c}
%     \toprule
%       \textbf{Model Family} & \textbf{\makecell[c]{Convolution\\Micro-level Aggregation}} & \textbf{Macro-level Aggregation} \\
%     \midrule
%         Homogenization & \multirow{3}{*}{\makecell[c]{GCNConv, GATConv\\ SageConv, GINConv}}  &  -\\
%     \midrule
%         Relation & & \multirow{2}{*}{\makecell[c]{Mean, Max\\ Sum, Attention }} \\
%     \midrule
%         Meta-path \\
%         % \makecell[c]{Convolution \\ Micro-level Aggregation} & GCNConv, GATConv, SageConv, GINConv\\
%         % Macro-level Aggregation & Mean, Max, Sum, Attention \\
%     \bottomrule
%     \end{tabular}}
%     \label{tab:model families}
%     \end{center}
% \end{table}
\begin{table}[h]
    \caption{Unique design dimensions in HGNNs}
    \begin{center}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c}
    \toprule
       \textbf{Design Dimension} & \textbf{Choices} \\
    \midrule
        Model Family & Homogenization, Relation, Meta-path \\
    \midrule
        \makecell[c]{Micro-level Aggregation \\ (Graph Convolution Layer)} & GCNConv, GATConv, SageConv, GINConv\\
    \midrule
        Macro-level Aggregation & Mean, Max, Sum, Attention \\
    \bottomrule
    \end{tabular}}
    \label{tab:model families}
    \end{center}
\end{table}
\subsubsection{\textbf{The Homogenization Model Family}}
The homogenization model family uses the direct-aggregation combined with any graph convolutions. Here we use the term \emph{homogenization} because all HGNNs included here apply direct-aggregation after the homogenization of the heterogeneous graph mentioned in Section~\ref{HG transformation}. Homogeneous GNNs and heterogeneous variants of GAT mentioned in Section~\ref{Hmp-aggregation} all fall into this model family. The homogeneous GNNs are usually evaluated as basic baselines in HGNN papers. Feeding the original graph into the homogeneous GNNs by ignoring the heterogeneity of nodes/edges is reasonable intuitively. Though it losses type information, it is confirmed that the simple homogeneous GNNs can outperform some existing HGNNs \cite{Simple-HGN}, which means they are nonnegligible and supposed to be seen as a model family. We select four graph convolutions from respective to the original model, which are GraphConv \cite{GCN}, GATConv \cite{GAT}, SageConv-mean \cite{sage} and GINConv\cite{GIN} as analyzed candidates.
% The heterogeneous variants of GAT are included here but they are not choices in convolution dimension since it cannot be used in the other two paradigms.  
% \quan{Do you mean our experiments did not cover all those variants?  If we extend the convolution modules to include those attentions then they will be covered, right?  If so, we can phrase it that way, like "The heterogeneous variants of GAT also fall into this category with appropriate convolution modules."}

\subsubsection{\textbf{The Relation Model Family}}
The model family applies relation subgraph extraction and dual-aggregation. The first HGNN model RGCN \cite{RGCN} is a typical example in relation model family, whose dual-aggregation consists of a micro-level aggregation with SageConv-mean and macro-level aggregation of Sum.  HGConv \cite{HGConv} is a combination of GATConv and attention. We could get other designs by enumerating the combinations of micro-level and macro-level aggregation.  In our experiments, we set the micro-level aggregations the same as graph convolutions in the homogenization model family, and macro-level aggregations are chosen among Mean, Max, Sum, and Attention.
%So we could get a number of designs through flexible combination of mirco-level and macro-level aggregation. Here the micro-level aggregation is consistent with convolution in homogeneous paradigm. The candidate macro-level aggregations are mean, max, sum and attention.
% \quan{Noticed that you frequently have "And" as the first word of a sentence.  This is not necessary.}

\subsubsection{\textbf{The Meta-path Model Family}}
The model family applies meta-path subgraph extraction and dual-aggregation. The instance HAN \cite{HAN} has the same dual-aggregation with HGConv \cite{HGConv} in the relation model family but different subgraph extraction. The candidate of micro-level and macro-level aggregations is the same as those in the relation model family.
% The HGNNs based on meta-path utilize the semantic information well and show great performance. However, the meta-path selection needs human prior and \cite{Simple-HGN} concludes that meta-paths are not necessary in most heterogeneous datasets. 
% \quan{We don't have to talk about how authors and other people judge metapath-based GNNs, meaning that the previous two sentences are unnecessary.  You can just say (how) HAN falls into this paradigm.} 
% Here we hope to report comprehensive analysis whether the HGNNs based on meta-paths with various dual-aggregation combination make progress.  \quan{This sentence is also not necessary.} 

\subsection{Space4HGNN: Platform for Design Space in HGNN} \label{space4hgnn}
We developed Space4HGNN, a novel platform for exploring HGNN designs. We believe Space4HGNN can significantly facilitate the research field of HGNNs. It is implemented with PyTorch~\footnote{\url{https://pytorch.org/}} and DGL~\footnote{\url{https://github.com/dmlc/dgl}}, using the OpenHGNN~\footnote{\url{https://github.com/BUPT-GAMMA/OpenHGNN}} package. It also offers a standardized evaluation pipeline for HGNNs, much like \cite{you2020design} for homogeneous GNNs. For faster experiments, we offer parallel launching. Its highlights are summarized below.

\subsubsection{\textbf{Modularized HGNN Implementation}}
The implementation closely follows the GNN design space GraphGym. It is easily extendable, allowing future developers to plug in more choices of design dimensions (e.g., a new graph convolution layer or a new macro-aggregation). Additionally, it is easy to import new design dimensions to Space4HGNN, such as score function in link prediction.

\subsubsection{\textbf{Standardized HGNN Evaluation}}
Space4HGNN offers a standardized evaluation pipeline for diverse architecture designs and HGNN models. Benefiting from OpenHGNN, we can evaluate diverse datasets in different tasks easily and offer visual comparison results presented in Section~\ref{experiments}.



==> Input/Evaluation.tex <==
\section{Evaluation Settings}
Our design space could be viewed as a hyper-parameter space. Compared with neural networks configured by a pure grid search, \cite{bergstra2012random} find that random search over the same domain is able to find models that are as good or better within a small fraction of the computation time. If we could know ahead of time which sub-spaces would be important, then we could design an appropriate grid. According to that, we have an attempt to find out the importance of different dimensions. To discover guidelines on how to design and apply HGNNs, here we want to answer the following specific questions:

\begin{itemize}
    \item In common design with GNNs, how to distill in sights from the huge number of dimension combination and condense design space to get an effective HGNN ?
    \item Which model family outperforms than others?
    \item Which component plays an important role in HGNNs?
\end{itemize}

\subsection{Uniform random search}\label{Uniform random search}
To answer the first question, we propose simple uniform random search by following up \cite{you2020design}. The unique design in HGNNs is more essential than other common design and we aim to analyze three model families comprehensively.
First, we analyze the dimensions of common design with GNNs. Take BatchNorm (BN) as example, we first draw S random experiments from the 10M possible combinations. We set S=24 and control every model family has 8 hits uniformly. And the four convolutions in each model family have 2 random hyper-parameters. Second, we condense HGNN design space and analyze the model families. And we perform a grid search for the condensed HGNN design space.

\subsection{Comparison Method}
\label{eva:comp}
We will conduct a comprehensive analysis of the performance of different designs. Different comparison methods provide different perspectives for our analysis. Here we adopt some common comparison methods like point estimates for model, curve estimates and distribution estimates for design space.

\subsubsection{\textbf{Point Estimates}}
Most recent works on HGNNs usually compare models with \textbf{point estimates} which compares the best performance of models in specific setting, often irrespective of model complexity. As shown in Table~\ref{tab:NC_performance}, reporting the best performance is an important way to measure the quality of the model.

\subsubsection{\textbf{Ranking Estimates}}
We usually also pay attention to the correlation between model performance and hyper-parameters, e.g. hyper-parameter sensitivity analysis. We can draw a curve to analyze the relation between performance with complexity or something whose value is usually continuous or ordinal. A tracking curve can describe the relationship between performance and complexity. However, the trend of a curve cannot accurately describe the categorical hyper-parameters. Ranking analysis proposed in \cite{you2020design} is another way to measure the impact of hyper-parameters whose value can be discrete. As shown in Fig.~\ref{fig:rank}, the rank analysis shows the ranking value of different choices in each dimension.

\subsubsection{\textbf{Distribution Estimates}}
\cite{radosavovic2019network} proposes a new comparison paradigm of distribution estimates. And different design spaces can be compared with a distribution curve as shown in Fig ~\ref{fig:gnn_type_dis}. To compare distributions, we use empirical distribution functions (EDFs). Let $\mathbf{1}$ be the indicator function. Given a set of $n$ models with scores{$s_{i}$}, the score EDF is give by:

\begin{equation}
F(e)=\frac{1}{n} \sum_{i=1}^{n} \mathbf{1}\left[s_{i}<s\right]
\end{equation}

$F(e)$ gives the fraction of models with score less than $s$. In our design space, each model family corresponds to a subspace and can be compared by distribution estimate.

% \label{rank_analysis}
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{images/loss_fn.png}
%     \caption{Loss function between DistMult and dot product. The left is rank analysis and the right is distribution estimates (curves in top figures are 24 experimental setups and the bottom is plotted in all thousands of setups.}
%     \label{fig:loss_fn}
% \end{figure}
% The rank analysis proposed by \cite{you2020design} is not suitable for our requirements. We take score function in link prediction as example. Compared to the commonly used dot product, HGB \cite{Simple-HGN} finds DistMult~\cite{yang2014embedding} outperforms dot product sometimes even when there is only single type of edge to predict. Based on our design space, we compare the HGNN performance with dot product or DistMult as the scoring function for the link prediction task using the uniform random search. The results are shown in Fig.~\ref{fig:loss_fn}, the left rank analysis shows dot product is better choice from bar plot and violin plot, which is not consistent with the claim in ~\cite{Simple-HGN}. The right distribution estimate shows more detailed statistics about performance score. We surprisingly observe that the DistMult overtake in a position of higher performance.

\subsection{Computational budget}
The novel controlled random search technique from \cite{you2020design} controls the number of trainable parameters by adjusting the hidden dimension. However, to analyze the relation between trainable parameters with performance, here we select hidden dimension as a design dimension. We do not constrain the parameters of GNNs as long as the computation fits into GPU memory, and we ignore the experiments if they run out-of-memory (OOM), which is less than 1\%. All experiments are conducted on p2.8xlarge (AWS) with each experiment running on a single K80 GPU with 12GB memory, which should be available in most research organizations.


==> Input/Preliminary.tex <==

\section{Preliminary}

\subsection{Graph Neural Network}
Graph Neural Networks (GNNs) aim to apply deep neural networks to graph-structured data. Here we focus on message passing GNNs which could be implemented efficiently and proven great performance. 
\begin{definition}[Message Passing GNNs \cite{messagepssing}]
Message passing GNNs aim to learn a representation vector $\boldsymbol{h}_{v}^{(L)} \in \mathbb{R}^{d_{L}}$ for each node $v$ after $L$-th message passing layers of transformation, and $d_{L}$ means the output dimension in $L$-th message passing layer.
% Let $\boldsymbol{h}_{v} \in \mathbb{R}^{d}$ be the feature for node $v$. 
The message passing paradigm defines the following node-wise and edge-wise computation for each layer as:
\begin{equation}
\text { Edge-wise: } \mathbf{m}_{e_{i j}}^{(L+1)}=\phi\left(\mathbf{h}_{i}^{(L)}, \mathbf{h}_{j}^{(L)}\right), j \in \mathcal{N}_{i},
\end{equation}
% \quan{What is $w_e^{(L)}$?  You only defined $w_e$.}
where $\mathcal{N}_{i}$ means neighbors of node $v_i$, $\phi$ is a message function defined on each edge to generate a message by combining the features of its incident nodes, and $e_{i j}$ denotes an edge from node $v_j$ to $v_i$;

\begin{equation}
\text { Node-wise: } \mathbf{h}_{i}^{(L+1)}=\psi\left(\mathbf{h}_{i}^{(L)}, \rho\left(\left\{\mathbf{m}_{e_{i j}}^{(L+1)}: \forall{j} \in \mathcal{N}_{i}\right\}\right)\right),
\end{equation}
where $\mathcal{N}_{i}$ means neighbors of node $v_i$, $\psi$ is an update function defined on each node to update the node representation by aggregating its incoming messages using the aggregation function $\rho$.  
% \quan{The message set is wrong; it should only contain the neighbors, not the entire $\mathcal{E}$.}
\end{definition}
\textbf{Example:} GraphSAGE~\cite{sage} can be formalized as a message passing GNN, where the message function is $\phi = h_{j}^{(L)} W^{(L)}$ and the update function is $\psi = \operatorname{SUM}{\left(\{ \mathbf{m}_{e_{i j}}^{(L+1)}: \forall{j} \in \mathcal{N}_{i}\}\right)}$. 
% \quan{[Agree]Same problem.  Also for GCN you need to multiply messages with $1/\sqrt{d_i d_j}$.  Or you could replace the example with GraphSAGE.}

\subsection{Heterogeneous Graph}
\begin{definition}[Heterogeneous Graph]
A heterogeneous graph, denoted as  $\mathcal{G}=(\mathcal{V},\mathcal{E})$ , consists of a node set $\mathcal{V}$ and an edge set $\mathcal{E}$. A heterogeneous graph is also associated with a node type mapping function $f_{v}: \mathcal{V} \rightarrow \mathcal{T}^{v}$ and an edge type (or relation type) mapping function $f_{e}: \mathcal{E} \rightarrow \mathcal{T}^{e}$. $\mathcal{T}^{v}$ and $\mathcal{T}^{e}$ denote the sets of node types and edge types.
Each node $v_{i} \in \mathcal{V}$ has one node type $f_{v}\left(v_{i}\right) \in \mathcal{T}^{v}$. Similarly, for an edge $e_{i j} \in \mathcal{E}$ from node $i$ to node $j$, $f_e(e_{i j}) \in \mathcal{T}^e$.
% for an edge  $e_{i j} \in \mathcal{E}$ from node $i$ to node$j$, $f_{e}\left(e_{i j}\right) \in \mathcal{T}^{e}$. 
When $\left|\mathcal{T}^{v}\right|>1$ or $\left|\mathcal{T}^{e}\right|>1$, it is a heterogeneous graph, otherwise it is a homogeneous graph.  
% \quan{A few suggestions: (1) $\mathbf{X}$ is not used in the definition, while $\mathcal{T}^v, \mathcal{T}^e, f_v, f_e$ did not appear in the text before.  (2) The use of $\mathcal{E}$ is inconsistent: here it is a set of edges while in the above section it is a set of source-destination-edge triplets.  I would change this sentence to "for an edge $(i, j, e) \in \mathcal{E}$ from node $i$ to node $j$, $f_e(e) \in \mathcal{T}^e$.  (3) For prettiness and reference I would suggest you use \texttt{amsthm} package for writing definitions/theorems/etc.  See \url{https://www.overleaf.com/learn/latex/Theorems_and_proofs}.}
\end{definition}
\textbf{Example.} As shown in Figure~\ref{fig:architecture} (left), we construct a simple heterogeneous graph to show an academic network. It consists of multiple types of objects (Paper(P), Author (A), Conference(C)) and relations (written-relation between papers and authors, published-relation between papers and conferences).
\begin{definition}[Relation Subgraph] \label{relation subgraph}
A heterogeneous graph can also be represented by a set of adjacency matrices $\left\{A_{k}\right\}_{k=1}^{K}$, where $K$ is the number of edge types $\left|\mathcal{T}^{e}\right|$. $A_{k} \in \mathbf{R}^{n_s \times n_t}$ is an adjacency matrix where $A_{k}[i, j]$ is non-zero when there is an edge $e_{i j}$ with $k$-th type from node $v_{i}$ to node $v_{j}$. $n_{s}$ and $n_{t}$ are numbers of source and target nodes corresponding to the edge type $k$ respectively. A relation subgraph of $k$-th edge type is therefore a subgraph whose adjacency matrix is $A_k$.
% \quan{[Agree]A bit confusing here: an adjacency matrix is a subgraph?  You can say "A relation subgraph of edge type $k$ is therefore a subgraph whose adjacency matrix is $A_k$" (if I got it right).} 
As shown in Figure~\ref{fig:graph} (b), the underlying data structure of the academic network in Figure~\ref{fig:architecture} (left) consists of four adjacency matrices.
\end{definition}

\begin{definition}[Meta-path \cite{sun2011pathsim}]\label{MP}
A meta-path $\mathcal{P}$ is defined as a path in the form of $v_{1} \stackrel{r_{1}}{\longrightarrow} v_{2} \stackrel{r_{2}}{\longrightarrow} \cdots \stackrel{r_{l}}{\longrightarrow} v_{l+1}$ which describes a composite relation $r_{1} \circ r_{2} \circ \cdots \circ r_{l}$ between two nodes $v_{1}$ and $v_{l+1}$, where $r_{l} \in \mathcal{T}^{e}$ denotes the $l$-th relation type of meta-path and $\circ$ denotes the composition operator on relations.

\begin{definition}[Meta-path Subgraph] \label{mp_subg}
Given a meta-path $\mathcal{P}$, $r_{1} \circ r_{2} \circ \cdots \circ r_{l}$ , the adjacency matrix $A_{\mathcal{P}}$ can be obtained by 
a multiplication of adjacency matrices according relations as
\begin{equation}
\boldsymbol{A}_{\mathcal{P}}=\boldsymbol{A}_{r_{1}} \ldots \boldsymbol{A}_{r_{l-1}} \boldsymbol{A}_{r_{l}}.
\label{eq1}
\end{equation}
% \quan{It's better to split this into two definitions: meta-path (which you need to cite the original meta-path paper) and meta-path subgraph (also define it).}
\end{definition}
The notion of meta-path subsumes multi-hop connections and a \textbf{meta-path subgraph} is multiple relation subgraphs matrices multiplication shown in Figure~\ref{fig:graph} (b) (iii). So relation subgraph is a special case of meta-path subgraph which is only composited by a relation subgraph. When meta-path beginning node type and ending node type are the same, meta-path subgraph is a homogeneous graph, otherwise a bipartite graph. 
% \quan{A meta-path subgraph is not really a composition of multiple subgraphs, so this paragraph is inaccurate.  I will just remove it though, and simply say "Note that relation subgraph is a special case of meta-path subgraph" and stop.}
\end{definition}

% \begin{table}[htbp]
% \caption{Table Type Styles}
% \begin{center}
% \begin{tabular}{|c|c|c|c|}
% \hline
% \textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
% \cline{2-4} 
% \textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
% \hline
% copy& More table copy$^{\mathrm{a}}$& &  \\
% \hline
% \multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
% \end{tabular}
% \label{tab1}
% \end{center}
% \end{table}

\subsection{Heterogeneous Graph Neural Network}\label{pre-HGNN}
Different from GNNs, HGNNs need to handle the heterogeneity of structure and capture rich semantics of heterogeneous graphs. According to the strategies of handling heterogeneity, HGNN can be roughly classified into two categories: HGNN based on one-hop neighbor aggregation (similar to traditional GNN) and HGNN based on meta-path neighbor aggregation (to mine semantic information), shown in Table~\ref{tab:model}.

\subsubsection{\textbf{HGNN based on one-hop neighbor aggregation}} 
To deal with heterogeneity, this kind of HGNN usually contains type-specific convolution. Similar to GNNs, the aggregation procedure occurs in one-hop neighbors. As earliest work and an extension of GCN \cite{GCN}, RGCN \cite{RGCN} assigns different weight matrices to different relation types and aggregates one-hop neighbors. With many GNN variants appearing, homogeneous GNNs inspire more HGNNs and then HGConv \cite{HGConv} dual-aggregate one-hop neighbors based on GATConv \cite{GAT}. A recent work SimpleHGN \cite{Simple-HGN} designs relation-type weight matrices and embeddings to characterize the heterogeneous attention over each edge. Besides, some earlier models, like HGAT \cite{HGAT}, HetSANN \cite{HetSANN}, HGT\cite{HGT}, modify GAT \cite{GAT} with heterogeneity by assigning heterogeneous attention for either nodes or edges. 
% \quan{Here we only talk about "one-hop aggregation", so I don't think you need to talk about direct- and dual-aggregation here; you can say that in Section 4.3.}

\begin{figure*}[htpb]
    \centering
    \includegraphics[width=\textwidth]{images/graph.png}
    \caption{
    The detailed description of three components using the graph illustrated in Figure~\ref{fig:architecture}.
    (a) \emph{Heterogeneous Linear Transformation} maps all node features to a shared feature space.
    % (b) Feature preprocessor: the features of different nodes with no feature or different dimension features will be mapped to a shared feature space. 
    (b) \emph{Heterogeneous Graph Transformation} (The left one) The original graph consists of four adjacency matrices representing four relations. (The right four) Four transformation methods.
    (c) Two aggregation methods in \emph{Heterogeneous Message Passing Layer}. (The left one) The direct-aggregation: lines assigned normalized attention coefficients indicate aggregation procedure. (The right one) The dual-aggregation: the black solid line indicates the micro-level aggregation procedure applied in different subgraphs and the thick red solid lines indicates the macro-level aggregation procedure.}
    % (d) Two heterogeneous aggregation methods. (i) The direct-aggregation:  dotted lines assigned normalized attention coefficients indicates aggregation procedure. (ii) The dual-aggregation: the black solid line indicates the micro-level aggregation procedure and the thick red solid lines indicates the macro-level aggregation procedure.}
    % \quan{A few suggestions.  (1) In the figures you can just say $A_{PA}$ instead of "relation subgraph: PA" which (i) saves more space, and (ii) can more easily align to each matrix.  Also, for the first occurrence of caption "Meta-path subgraph: PAP" I would rather say "$A_{PAP} = A_{PA} A_{AP}$" instead, which explicitly says how the meta-path subgraphs are constructed.  The second "Meta-path subgraph: PAP" can be replaced with $A_{PAP}$ since you already said before how to compute it.  (2) I don't think putting feature preprocessor in the figure is necessary, as it is not directly related to our new design space dimensions, especially since Table 1 and Table 4 never talked about it.  (3) I would rather have two aggregation methods separated in the figure (with one taking the place of feature preprocessor).}
    \label{fig:graph}
\end{figure*}

\subsubsection{\textbf{HGNN based on meta-path neighbor aggregation}}Another class of HGNNs is to capture higher-order semantic information with hand-crafted meta-paths. Different from the previous, aggregation procedure occurs in neighbors connected by meta-path. As a pioneering work, HAN \cite{HAN} first uses node-level attention to aggregate nodes connected by the same meta-path and utilizes semantic-level attention to fuse information from different meta-paths. Because the meta-path subgraph ignores all the intermediate nodes, MAGNN \cite{MAGNN} aggregates all nodes in meta-path instances to ensure that information will not be missed. Though meta-paths contain rich semantic information, the selection of meta-paths needs human prior and determines the performance of HGNNs. Some works like GTN \cite{GTN} learn meta-paths automatically to construct a new graph. HAN \cite{HAN} and HPN \cite{HPN}, which are easy to extend, will be included in our framework for generality. 
%   \quan{Here we only talk about "meta-path aggregation", so this two-stage-thing-a-majig can also be moved to Section 4.3.  Instead, you should emphasize the aspect that HAN constructs a meta-path subgraph.  Afterwards you can say "because meta-path subgraph ignores all the intermediate nodes, MAGNN aggregates..."}


\subsection{Model Evaluation and Design Space}
There are many works to measure progress in the field by evaluating models. The work \cite{dacrema2019we} reports the results of a systematic analysis of neural recommendation mentioning HGNNs and sheds light on potential problems. Several works \cite{errica2019fair, dwivedi2020benchmarking, shchur2018pitfalls} discuss how to make fair a comparison between GNN models. In HGNNs, a recent work \cite{Simple-HGN} revisits HGNNs and proposes issues with existing HGNNs. The above work is to evaluate models from the model-level sight. 

Though rigorous theoretical understanding of neural network is not enough, it is imperative to perform empirical studies of neural network to discover better architectures. In visual recognition, some works \cite{radosavovic2019network, radosavovic2020designing}design network design spaces to help advance the understanding of network design and discover design principles that generalize across settings. Inspired by that, GraphGym \cite{you2020design} proposes a GNN design space and a GNN task space to evaluate model-task combinations comprehensively. 

Here we aim to extensively explore the design space of HGNNs involving many design dimensions and evaluate different design architectures. Different from the model-level sight of \cite{Simple-HGN}, we evaluate the design dimensions from module-level sight and distill helpful design principles. Different from GraphGym \cite{you2020design}, our design space focuses on the unique design dimension of HGNNs and explores the differences with GNNs. 
% \quan{After scanning the paper I'm wondering if we need to have a dedicated section talking about model evaluation (especially in main text). A dedicated section will easily distract readers making them think that our work proposes some new way of evaluating GNNs (which is not the case).}

% \cite{shchur2018pitfalls} shows that results are highly dependent on the particular train/ validation/ test split, and different splits result in different performance rankings dramatically.

% Recently neural architecture search(NAS) in GNNs achieves great performance without handcrafted hyper-parameter tuning \cite{guan2021autogl, autognn, graphnas}. 
% Neural architecture search (NAS) generally contains two crucial components: a network search space and a search algorithms over that space. Design space is a complement of NAS and mainly concerns the search space. Besides, NAS usually aims to find the single best model and design space focus on characterizing the model family \cite{radosavovic2019network}. AutoGNN \cite{autognn} and GraphNAS \cite{graphnas} employ automatic search to find an optimal GNN architecture. GraphGym \cite{you2020design} proposes a GNN design space and a GNN task space to evaluate model-task combinations comprehensively. In HGNNs, \cite{diffmg} design an expressive search space in the form of a directed acyclic graph(DAG), which focuses on meta-path and may not cover most HGNNs. Here we define design space for HGNN, which can be the basis of NAS for HGNN.
% \begin{table*}
%   \caption{HGNN models category}
%   \begin{tabular}{l|c|c|c|c}
%     \toprule
%         \textbf{Neighbors} & \multicolumn{3}{c|}{\textbf{One-hop}}  & \textbf{Meta-path }  \\
%     \midrule
%         \textbf{Aggregation} & \makecell[c]{Homogeneous \\ Direct-aggregation} & \makecell[c]{Heterogeneous \\Direct-aggregation} & \multicolumn{2}{c}{Dual-aggregation} \\
%     \midrule
%         \textbf{Message} & Type-agnostic & \multicolumn{3}{c}{Type-specific} \\
%     \midrule
%         \textbf{Reduce} & \multicolumn{2}{c|}{direct} & \multicolumn{2}{c}{Type-specific} \\
%     \midrule
%         \textbf{Paradigm} & - & Homogeneous paradigm & Relation paradigm & Meta-path paradigm\\
%     \midrule
%         \textbf{Target Graph} & \multicolumn{2}{c|}{\makecell[c]{Whole graph \\ Direct-aggregation}} & \multicolumn{2}{c}{\makecell[c]{Subgraph conv first\\ the aggregation cross type}} \\
%     \midrule
%         \textbf{Conv} & heterogeneous conv & \multicolumn{3}{c}{homogeneous conv} \\
%     \midrule
%         \textbf{Macro-level} & \multicolumn{2}{c|}{None} & \multicolumn{2}{c}{Mean-Sum-Max} \\
%     \midrule
%         \textbf{Model} & \makecell[c]{HGAT\cite{HGAT} HetSANN\cite{HetSANN} \\HGT\cite{HGT} Simple-HGN\cite{Simple-HGN}} & 
%         \makecell[c]{GCN\cite{GCN} GAT\cite{GAT} \\ GraphSage\cite{sage} GIN\cite{GIN}}& 
%         RGCN\cite{RGCN} HGConv\cite{HGConv} & 
%         HAN\cite{HAN} HPN\cite{HPN} \\
%     \bottomrule
%   \end{tabular}
% \label{tab:model category}
% \end{table*}
%
% Receptive    | One-hop                            | Meta-path          |   (Not a dimension)
% Aggregation  | Direct                 | Dual                           |
% Message      | Homogeneous | Relation-specific    | Meta-path-specific |
% Model        | GAT...      | HGAT...  | RGCN...   | HAN...             |
%
% GCN: a1 = x1 @ W, a2 = x2 @ W, .....m, paper = sum(a1..a5)
% RGCN: a1 = x1 @ Wap, a2 = x2 @ Wap, a3 = x3 @ Wpap, ..., paper=sum(sum(all ap), sum(all pap))
